Knowledge Connectivity Requirements for Solving BFT Consensus with Unknown Participants and Fault Threshold (Extended Version)

Consensus stands as a fundamental building block for constructing reliable and fault-tolerant distributed services. The increasing demand for high-performance and scalable blockchain protocols has brought attention to solving consensus in scenarios where each participant joins the system knowing only a subset of participants. In such scenarios, the participants' initial knowledge about the existence of other participants can collectively be represented by a directed graph known as knowledge connectivity graph. The Byzantine Fault Tolerant Consensus with Unknown Participants (BFT-CUP) problem aims to solve consensus in those scenarios by identifying the necessary and sufficient conditions that the knowledge connectivity graphs must satisfy when a fault threshold is provided to all participants. This work extends BFT-CUP by eliminating the requirement to provide the fault threshold to the participants. We indeed address the problem of solving BFT consensus in settings where each participant initially knows a subset of participants, and although a fault threshold exists, no participant is provided with this information -- referred to as BFT Consensus with Unknown Participants and Fault Threshold (BFT-CUPFT). With this aim, we first demonstrate that the conditions for knowledge connectivity graphs identified by BFT-CUP are insufficient to solve BFT-CUPFT. Accordingly, we introduce a new type of knowledge connectivity graphs by determining the necessary and sufficient conditions they must satisfy to solve BFT-CUPFT. Furthermore, we design a protocol for solving BFT-CUPFT.

==> temp/temp-main <==
\input{packages}

\begin{document}
\title{
    {\huge Knowledge Connectivity Requirements for Solving BFT Consensus with Unknown Participants and Fault Threshold}
}

\author{
\IEEEauthorblockN{} 

\IEEEauthorblockA{LASIGE, Faculdade de Ciências, Universidade de Lisboa, Portugal}

\{\}@ciencias.ulisboa.pt
}

\maketitle

\begin{abstract}
    Consensus stands as a fundamental building block for constructing reliable and fault-tolerant distributed services. 
    The increasing demand for high-performance and scalable blockchain protocols has brought attention to solving consensus in scenarios where each participant joins the system knowing only a subset of participants.
    In such scenarios, the participants' initial knowledge about the existence of other participants can collectively be represented by a directed graph known as \textit{knowledge connectivity graph}. 
    The \textit{Byzantine Fault Tolerant Consensus with Unknown Participants} (BFT-CUP) model aims to solve consensus in those scenarios by identifying the necessary and sufficient conditions that the knowledge connectivity graphs must satisfy when a fault threshold is provided to all participants.
    This work extends the BFT-CUP model by eliminating the requirement to provide the fault threshold to the participants.
    We indeed address the problem of solving BFT consensus in settings where each participant initially knows a subset of participants, and although a fault threshold exists, no participant is provided with this information~--- referred to as \textit{BFT Consensus with Unknown Participants and Fault Threshold} (BFT-CUPFT).
    With this aim, we first demonstrate that the conditions for knowledge connectivity graphs identified by the BFT-CUP model are insufficient to solve BFT-CUPFT.
    Accordingly, we introduce a new type of knowledge connectivity graphs by determining the necessary and sufficient conditions they must satisfy to solve BFT-CUPFT.
    Furthermore, we design a protocol for solving BFT-CUPFT.  
\end{abstract}

\begin{IEEEkeywords}
    Consensus with Unknown Participants, Byzantine Fault-Tolerant Consensus, Blockchain.
\end{IEEEkeywords}

\section{Introduction}
\noindent\textbf{Context.} Consensus is a fundamental building block for constructing fault-tolerant and strongly consistent distributed systems where participants agree on a common value out of the initially proposed values.
This problem has been primarily addressed in three settings~-- permissioned, permissionless, and hybrid.
In the permissioned setting, participants have a single global view of the system in advance, i.e., each process is provided with the \textit{system's membership} and the \textit{fault threshold} (or, more generally, the fail-prone system~\cite{malkhi_1998}). 
Knowing such parameters simplifies the design and analysis of consensus protocols.
%Although the protocols designed for this setting (e.g., PBFT~\cite{castro_1999}) are high-performance, they suffer from scalability issues, primarily due to the significant number of message exchanges~\cite{vukolic_2015,hotstuff}.

In the permissionless setting, protocols such as the Nakamoto consensus used in Bitcoin~\cite{nakamoto_2008} solve consensus without requiring a single global view of the system.
Specifically, no participant might be aware of the set of all participants.
Furthermore, the fault threshold is not explicitly defined in the same way as in the permissioned setting; instead, these protocols rely on assumptions about the overall distribution of resources within their networks, like computational power in Bitcoin.
Despite these protocols being scalable in terms of the number of participants, their performance is significantly lower by orders of magnitude compared to consensus protocols designed for the permissioned setting~\cite{vukolic_2015,korkmaz2022alder, Cachin2017BlockchainCP}.

The demand to scale consensus to accommodate numerous participants while maintaining high performance gave rise to the hybrid setting. 
Protocols tailored for this setting relax the global view requirements found in permissioned consensus, enabling each participant to have a partial view of the participants it can trust or initially knows.
Protocols designed for this setting can be modeled in various ways. 
One approach is through the use of consensus with unknown participants~\cite{cavin_2004, cavin_2005, greve_2007, alchieri_2016,khanchandani_2021, vassantlal_2023}. Alternatively, federated Byzantine quorum systems~\cite{lokhava_2019,garcia_2018,mazieres_2015,garcia_2019}, personal Byzantine quorum systems~\cite{losa_2019}, quorum systems designed for permissionless networks~\cite{cachin_2022}, and heterogeneous quorum systems~\cite{li2023quorum} offer additional modeling options for hybrid consensus protocols.
This paper focuses on the model of consensus with unknown participants.

\vspace{0.5em}
\noindent\textbf{Consensus with unknown participants.}
In scenarios where each participant joins the network initially knowing only a subset of other participants, participants' knowledge about the existence of other participants can collectively be represented by a directed graph known as \textit{knowledge connectivity graph}~\cite{cavin_2004}.
In such graphs, each vertex represents a participant, and a directed edge from vertex~$i$ to another vertex~$j$ denotes that participant~$i$ initially knows participant~$j$.
The graph depicted in Fig.~\ref{fig:osr:example:impossible} is an example of a knowledge connectivity graph in which participant~$1$ initially knows participants $2$, $3$, and $4$.
It is crucial to emphasize that \textit{a knowledge connectivity graph differs from a communication network}, as a participant~$i$ may be capable of communicating with another participant $j$; however, such communication cannot happen when $i$ lacks knowledge about the existence of $j$ (i.e., there is no link from $i$ to $j$ in their knowledge connectivity graph).

Given a knowledge connectivity graph, participants might be unable to solve consensus. 
For instance, in the graph depicted in Fig.~\ref{fig:osr:example:impossible}, if participant~$4$ is faulty and others are correct, correct participants cannot solve consensus as two subsets of participants~-- $\{1,2,3\}$ and $\{5,6,7,8\}$~-- are unable to achieve a state where mutual knowledge about each other is established.
The Consensus with Unknown Participants~(CUP) model explores the \textit{necessary and sufficient} properties that a knowledge connectivity graph must have to solve consensus under specific synchrony and fault assumptions. 
In this model, when joining the network, each participant is provided with the system's fault threshold in addition to knowing a subset of other participants~\cite{cavin_2004}.
Each participant's knowledge about the existence of other participants is encapsulated in a local oracle known as a \textit{participant detector}~(PD). 

The CUP model was studied across various settings, each characterized by distinct fault and synchrony assumptions~\cite{cavin_2004, cavin_2005, greve_2007, alchieri_2016}.
Given a knowledge connectivity graph, the knowledge of a participant increases (i.e., the number of its outgoing edges increases) with the relaxation of synchrony assumptions and the strengthening of fault assumptions.
For example, each participant in the Byzantine Fault-Tolerant~(BFT)~CUP~\cite{alchieri_2016} requires more knowledge than in the fault-free CUP model~\cite{cavin_2004}.   
The graph depicted in Fig.~\ref{fig:osr:example:possible} illustrates an example of a knowledge connectivity graph that satisfies the requirements of the BFT-CUP model.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \includegraphics[scale=0.8]{figures/osr-example-imp.pdf}
        \caption{A knowledge connectivity graph that does not satisfy the requirements of the BFT-CUP model. 
        Even though the number of Byzantine processes is less than one-third of the total processes, satisfying the requirement for solving the traditional Byzantine consensus~\cite{dwork_1988}, solving consensus in this system is impossible as participants in $\{1, 2, 3\}$ cannot acquire knowledge about participants in $\{5, 6, 7, 8\}$, and vice versa when the Byzantine participant remains silent.}
        \label{fig:osr:example:impossible}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \includegraphics[scale=0.8]{figures/osr-example.pdf}
        \caption{A knowledge connectivity graph that satisfies the requirements of the BFT-CUP model; hence, participants can solve consensus even in the presence of a Byzantine participant.}
        \label{fig:osr:example:possible}
    \end{subfigure}
    \caption{Two knowledge connectivity graphs.
    In each graph, a vertex corresponds to a participant, and the outgoing edges from a vertex point to the participants that the corresponding participant initially knows; for instance, participant $1$ initially knows participants $2$, $3$, and $4$.
    Participant~$4$ is Byzantine, and others are correct.}
    \label{fig:osr:examples}
\end{figure}

\vspace{0.5em}
\noindent\textbf{Problem statement.}
The BFT-CUP model solves consensus in partially synchronous systems, where each participant initially knows the system's global fault threshold and a subset of participants determined by its PD.
Since knowing the global fault threshold restricts the full potential of the BFT-CUP model in the hybrid setting, in this paper, we propose \textit{BFT Consensus with Unknown Participants and Fault Threshold} (BFT-CUPFT) model that eliminates the explicit knowledge of that parameter.
The BFT-CUPFT model is an extension of the BFT-CUP model that enables participants to solve Byzantine consensus where each participant initially knows a subset of participants.

\vspace{0.5em}
\noindent\textbf{Contributions.}
The main objective of this paper is to present a BFT consensus protocol in the hybrid model for the partially synchronous systems where each process is initialized only with the PD oracle, providing information about a subset of processes in the system without knowing the system's membership or the fault threshold.

With this aim, we begin by revisiting the BFT-CUP model under the extra assumption that each process can leverage digital signatures 
% \begin{enumerate*}[label=(\alph*)]
%     \item , and 
%     \item no process can add new processes to the set received from its PD
% \end{enumerate*}
(this assumption has been made in related work~\cite{garcia_2018,mazieres_2015,vassantlal_2023}).
We refer to the resulting model as the \textit{authenticated BFT-CUP} model.
% Besides, in practice, incorporating a proof-of-work requirement for each link in the knowledge connectivity graph can ensure that no process can augment the set received from its PD by adding new processes.
Notably, Alchieri et al.~\cite{alchieri_2008} established that the requirements of knowledge connectivity graphs for solving consensus in the BFT-CUP model remain unchanged, irrespective of whether digital signatures are taken into account.
Although such an assumption does not reduce the initial knowledge required by participants to solve consensus, it enables the design of a simpler consensus protocol.
We use the simpler protocol to highlight the significance of the fault threshold in the BFT-CUP model and clarify the necessary adjustments required when processes lack such information.

We then show an impossibility result stating that solving consensus is impossible in a partially synchronous system where the knowledge connectivity graph formed collectively by participants' PDs satisfies the requirements of the BFT-CUP model, yet no process is provided with the fault threshold. 
This holds even when considering the aforementioned extra assumption.
As a result, we introduce the \textit{BFT Consensus with Unknown Participants and Fault Threshold} (BFT-CUPFT) model, defining a new type of knowledge connectivity graphs in which participants can solve consensus without having information about the fault threshold.
Table~\ref{tbl} outlines the (im)possibility of solving Byzantine consensus deterministically under different system models.
Finally, we design a protocol to solve consensus on the BFT-CUPFT model.

In summary, the main contributions of this paper can be outlined as follows:
\begin{itemize}
    \item We revisit the BFT-CUP model by assuming that each process has access to digital signatures.
    We design protocols that are simpler than the original ones under this new assumption.
    \item We prove an impossibility result for solving consensus when knowledge connectivity graphs satisfy the requirements of the BFT-CUP model, but participants are not provided with the fault threshold. 
    \item We introduce the BFT-CUPFT model by defining a new type of knowledge connectivity graphs that allow participants to solve consensus when each participant initially knows only a subset of participants, not the system's membership or the fault threshold. 
    \item We design a consensus protocol that solves consensus in the BFT-CUPFT model.
\end{itemize}

\begin{table*}[t!]
\centering
\begin{tabular}{cl|cll|}
\cline{3-5}
\multicolumn{2}{c|}{\multirow{2}{*}{}} & \multicolumn{3}{c|}{\rule[-1ex]{0pt}{3.5ex}Knowledge about $n$ and $f$} \\ \cline{3-5} 
\multicolumn{2}{c|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Known $n$, Known $f$\end{tabular}} & \multicolumn{1}{l|}{\rule[-1ex]{0pt}{3.5ex}\begin{tabular}[c]{@{}l@{}}Unknwon $n$, Known $f$\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Unknown $n$, Unknown $f$\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Communication\\ Model\end{tabular}}} & Sync. & \multicolumn{1}{l|}{\rule[-1ex]{0pt}{3.5ex}\ding{51} (e.g.~\cite{abraham2017brief})} & \multicolumn{1}{l|}{\ding{51} (e.g.~\cite{khanchandani_2021})} & \multicolumn{1}{l|}{\ding{51} (e.g.~\cite{khanchandani_2021})} \\ \cline{2-5} 
\multicolumn{1}{|c|}{}  & \begin{tabular}[c]{@{}l@{}}\rule[-1ex]{0pt}{3.5ex}Partially Sync.\end{tabular} & \multicolumn{1}{l|}{\ding{51} (e.g.~\cite{castro_1999,hotstuff})} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}} \ding{51} (BFT-CUP~\cite{alchieri_2008,alchieri_2016})\end{tabular}} & \begin{tabular}[c]{@{}l@{}}{\color{teal} \ding{51} (BFT-CUPFT) $\leftarrow$ this work}\end{tabular} \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & Async. & \multicolumn{1}{l|}{\rule[-1ex]{0pt}{3.5ex}\ding{55} (see~\cite{flp})} & \multicolumn{1}{l|}{\ding{55} (see~\cite{flp})} & \multicolumn{1}{l|}{\ding{55} (see~\cite{flp})} \\ \hline
\end{tabular}
\caption{The (im)possibility of solving Byzantine consensus deterministically under different system models.}
\label{tbl}
\end{table*}

\vspace{0.5em}
\noindent\textbf{Paper organization.}
The remainder of the paper is organized as follows. 
Section~\ref{sec:preliminaries} introduces our system model and provides the background for this paper.
Section~\ref{sec:revisiting:bft:cup} revisits the BFT-CUP model by assuming that each process has access to digital signatures.
Section~\ref{sec:problem:specification} presents the problem specification and the impossibility result for solving consensus when knowledge connectivity graphs satisfy the requirements of the BFT-CUP model, but participants are not provided with the fault threshold.  
Section~\ref{sec:extended:bft:cup} introduces the BFT-CUPFT model, defining a new type of knowledge connectivity graphs. 
Section~\ref{sec:consensus:extended:bft:cup} solves consensus in the BFT-CUPFT model.
Section~\ref{sec:related:work} presents the related work.
Finally, Section~\ref{sec:conclusion} concludes the paper.

\section{Preliminaries}\label{sec:preliminaries}
\subsection{System Model}
We consider a distributed system comprised of a finite set~$\Pi$ of processes operating under the assumption of partial synchrony~\cite{chandra_1996, dwork_1988}, which guarantees that, for each execution of the protocol, there exists a time GST and a duration $\delta$ such that after GST, message delays between correct servers are bounded
by $\delta$. 
Prior to GST, messages may experience arbitrary delays.
We assume that each process~$i \in \Pi$ initially knows only a subset~$\Pi_{i} \subseteq \Pi$.

We denote the set of failed processes during an execution by $F \subset \Pi$.
The faulty processes can behave arbitrarily, i.e., can be Byzantine~\cite{lamport_1982}, and may collude and coordinate their actions.
A non-Byzantine process is said to be \textit{correct}.
We denote the set of correct processes during an execution by $C = \Pi \setminus F$.
We assume a static Byzantine adversary controlling the faulty processes, i.e., the set of processes controlled by the adversary is fixed at the beginning and does not change throughout the execution of the protocols.
We assume that correct processes neither know $\Pi$ nor $F$; however, Byzantine processes may know both.

We further assume that each process has a unique ID, IDs are not necessarily consecutive, and it is infeasible for a faulty process to obtain additional IDs to launch a \emph{Sybil attack} \cite{douceur_2002}.
Processes communicate by message passing through authenticated and reliable point-to-point channels, when needed, can sign messages using digital signatures. 
A process $i$ can only send a message directly to another process $j$ if $i$ knows $j$, i.e., if $j \in \Pi_{i}$. 

\subsection{The Consensus Problem} 
In the consensus problem, each process \emph{proposes} a value, and all correct processes must \emph{decide} the same value, which must be one of the proposed values. 
We focus on a variant of the Byzantine consensus problem that relies on an application-specific $\mathtt{valid}$ predicate to indicate whether a value is valid~\cite{makingByzConLive,cachin2001secure,crain2018dbft}. 
Assuming that each correct process proposes a valid value, each of them has to decide on a value so that the following properties are satisfied:
\begin{itemize}
    \item \emph{Validity:} a correct process decides on a valid value, i.e., satisfying $\mathtt{valid}$.
    \item \emph{Agreement:} all correct processes must decide the same value.
    \item \emph{Termination:} every correct process eventually decides some value.
\end{itemize}

\subsection{The BFT-CUP Model}
The \emph{Byzantine Fault-Tolerant Consensus with Unknown Participants} (BFT-CUP) model~\cite{alchieri_2016} solves consensus while tolerating Byzantine faults in partially synchronous systems.
The BFT-CUP model operates under the same system model as this paper, except it does not rely on digital signatures. 
It assumes every process is provided with the fault threshold~$f$ as input, providing an upper bound on the size of the faulty set $F$, i.e., $|F| \leq f$. 

In this model, each process initially obtains partial knowledge about the others using a distributed oracle called \emph{participant detector} (PD).
% Indeed, PD can be seen as an oracle providing hints about the system's participating processes.
In further detail, let $\mathit{PD}_i$ represent the local participant detector for process $i$, wherein $\mathit{PD}_i$ returns a set $\Pi_{i} \subseteq \Pi$ comprising the processes that $i$ can initially contact.
The information provided by the participant detectors of all processes collectively forms a directed graph known as the \emph{knowledge connectivity graph}~\cite{cavin_2004}. 
A directed graph $G_{\mathit{di}} = (V_{\mathit{di}}, E_{\mathit{di}})$ is a knowledge connectivity graph if $V_{\mathit{di}}$ represents the set of processes $\Pi$, and an edge $(i, j) \in E_{\mathit{di}}$ exists if and only if process~$i$ knows process~$j$, i.e., $j \in \mathit{PD}_i$.
For instance, the graphs illustrated in Fig.~\ref{fig:osr:examples} exemplify knowledge connectivity graphs wherein $\mathit{PD}_1 = \{2,3,4\}$.

It is essential to emphasize that the knowledge connectivity graph represents the list of processes that each process initially knows in the system, \textbf{not its network connectivity}.
Indeed, the network connectivity can be represented by a complete graph as there is a reliable point-to-point channel between any two processes, according to the system model. 
In further detail, when a process $i$ initially knows another process $j$, i.e., there is a directed link from $i$ to $j$ in the knowledge connectivity graph, process $i$ can send messages to $j$ from the beginning of the execution. 
However, when $j \notin \mathit{PD}_i$, process~$i$ first requires to discover $j$ through the processes it knows, and only after that it can directly communicate with $j$ using the reliable point-to-point channel between them.

The BFT-CUP model guarantees that processes can solve consensus when the knowledge connectivity graph meets specific requirements. 
Before delving into these requirements, we first review some relevant graph notations.
A directed graph $H_{\mathit{di}}=(V_{\mathit{di}},E_{\mathit{di}})$ is said to be \textit{$k$-strongly connected} if for any pair of nodes $i,j \in V_{\mathit{di}}$, $i$ can reach $j$ through at least $k$ node-disjoint paths in $H_{\mathit{di}}$.
The \textit{strong connectivity} $\kappa(H_{\mathit{di}})$ of $H_{\mathit{di}}$ is the maximum value of $k$ for which $H_{\mathit{di}}$ is $k$-strongly connected.
Given two non-empty sets of processes $A$ and $B$, we represent the existence of $k$ node-disjoint paths from any member of $A$ to any member $B$ by $A \xRightarrow[]{k} B$.
Besides, $A \xRightarrow[]{>k} B$ denotes that the number of node-disjoint paths from any member of $A$ to any member of $B$ is greater than $k$.

Given a directed graph $G_{\mathit{di}} = (V_{\mathit{di}}, E_{\mathit{di}})$, a component $G_{\mathit{sink}}$ of $G_{\mathit{di}}$ is a \emph{sink} if and only if there is no path from a node in $G_{\mathit{sink}}$ to other nodes of $G_{\mathit{di}}$, except nodes in $G_{\mathit{sink}}$ itself.
A node $v\in V_{\mathit{di}}$ is a \emph{sink member} if it belongs to a sink component of $G_{\mathit{di}}$; otherwise, it is a \emph{non-sink member}.
An undirected counterpart can be defined for any directed graph $G_{\mathit{di}}$ as $G = \boldsymbol{(}V_{\mathit{di}}, \{(i, j) \ | \ (i, j) \in E_{\mathit{di}} \lor (j, i) \in E_{\mathit{di}}\}\boldsymbol{)}$.
\begin{definition}[$k$-One Sink Reducibility ($k$-OSR) PD~\cite{alchieri_2016}]\label{def:osr}
A graph $G_{\mathit{di}}$ belongs to $k$-OSR PD if:
\begin{itemize}
    \item the undirected graph $G$ obtained from $G_{\mathit{di}}$ is connected,
    \item the directed acyclic graph obtained by reducing $G_{\mathit{di}}$ to its strongly connected components has exactly one sink, namely $G_\mathit{sink}=(V_\mathit{sink}, E_\mathit{sink})$,
    \item the sink component $G_\mathit{sink}$ is $k$-strongly connected, and
    \item there are at least $k$ node-disjoint paths from any process $i \notin V_\mathit{sink}$ to any process $j \in V_\mathit{sink}$.\qed
\end{itemize}    
\end{definition}
Given a knowledge connectivity graph $G_{\mathit{di}}=(V_{\mathit{di}},E_{\mathit{di}})$, an induced subgraph $G_{\mathit{safe}}$ is \textit{safe} if it is obtained by removing all Byzantine processes from $G_{\mathit{di}}$, i.e., $G_{\mathit{safe}}= \boldsymbol{(}V_{\mathit{di}}\setminus F, \{ (i,j) \ | \ i, j \in V_{\mathit{di}}\setminus F \land (i,j) \in E_{\mathit{di}}\}\boldsymbol{)}$. 
With these definitions, we are ready to present the requirements that a knowledge connectivity graph must satisfy to enable solving consensus in the BFT-CUP model.

\begin{theorem}[\hspace{-0.01em}\cite{alchieri_2016}]\label{thm:bft:cup}
The safe subgraph $G_{\mathit{safe}}$ of a knowledge connectivity graph must satisfy the following two properties to ensure correct processes can solve consensus in the BFT-CUP model:
\begin{itemize}
\item $G_{\mathit{safe}}$ belongs to the $(f+1)$-OSR PD, and
\item the sink component of $G_{\mathit{safe}}$ must contain at least $2f+1$ processes.\qed
\end{itemize}
\end{theorem}
If a knowledge connectivity graph meets the properties of Theorem~\ref{thm:bft:cup}, we say it satisfies the requirements of the BFT-CUP model.
We also denote the family of all finite graphs that meet these properties by $\mathcal{G}_{\mathit{di}}$.
Fig.~\ref{fig:osr:example:possible} is an example of a knowledge connectivity graph that satisfies the requirements of the BFT-CUP model in which participants in $\{1, 2, 3\}$ are the sink members of $G_{\mathit{safe}}$.

\vspace{0.5em}
\noindent\textbf{Solving consensus in the BFT-CUP model.}
The sink component holds a pivotal role in the BFT-CUP model. 
In order to solve consensus within this model, processes expand their knowledge~-- i.e., the set of processes they initially know~-- and actively seek to identify the sink component.
During this phase, processes communicate using a communication primitive called reachable reliable broadcast~\cite{alchieri_2016}.
This primitive allows delivery of a message if it is received through more than~$f$ node-disjoint paths from the sender.

Once the sink component is discovered, processes can establish intersecting quorums and execute a consensus protocol, such as PBFT~\cite{castro_1999}, on top of those quorums.
The definition of quorums highlights the significance of the sink: as demonstrated in~\cite{vassantlal_2023}, any defined quorum must include at least $\ceil{(|V_{\mathit{sink}}|+f+1)/2}$ sink processes to intersect with any other quorum in at least one correct process.
\begin{remark}
    The BFT-CUP model does not rely on digital signatures.\qed
\end{remark}

\section{Revisiting the BFT-CUP Model}\label{sec:revisiting:bft:cup}
This section revisits the BFT-CUP model, incorporating an additional assumption that allows each process to use digital signatures~-- denoting the resulting model as the \textit{authenticated BFT-CUP} model.
Recall that in the BFT-CUP model, a process delivers a message if it is received through more than $f$ node-disjoint paths.
However, using digital signatures, processes can deliver messages without waiting to receive them through multiple paths.
%However, using digital signatures, trusting the received messages does not require a protocol.
This substantially simplifies the communication protocols and reduces the places where the fault threshold is required.
As presented next, the consensus protocol in the authenticated BFT-CUP model has roughly 20 lines compared with 120 in \cite{alchieri_2016}.
Although the requirements of the knowledge connectivity graphs to solve consensus remain unchanged~\cite{alchieri_2008}, in the simplified protocol, we can highlight where the fault threshold is still required and clarify the necessary adjustments to remove it entirely.

% \subsection{The Authenticated BFT-CUP Model}
% The authenticated BFT-CUP model incorporates the original BFT-CUP model, assuming that 
% each process can leverage digital signatures.
% We initiate by demonstrating that a knowledge connectivity graph~$G_{\mathit{di}}$ must satisfy the requirements of the BFT-CUP model (i.e., $G_{\mathit{di}} \in \mathcal{G}_{\mathit{di}}$) in order to solve consensus in the revisited BFT-CUP model.
% \begin{theorem}\label{thm:verify:pd}
%     The requirements of the knowledge connectivity graphs to solve consensus in the revisited BFT-CUP model are the same as those of the BFT-CUP model. 
% \end{theorem}
% As the requirements of knowledge connectivity graphs for solving consensus remain unchanged, irrespective of whether processes can use digital signatures~\cite{alchieri_2008}, in order to prove the above theorem, we mainly need to demonstrate that the properties of the knowledge connectivity graphs outlined in Theorem~\ref{thm:bft:cup} remain unaffected when no process can add new processes to its initial knowledge.

\subsection{Consensus Protocol in the Authenticated BFT-CUP Model}
In order to solve consensus in the authenticated BFT-CUP model, we introduce three algorithms~-- namely Discovery, Sink, and Consensus~-- along with their associated properties. 
The relationship between these algorithms is as follows: the Consensus algorithm executes the Sink algorithm, and the Sink algorithm executes the Discovery algorithm.
These algorithms highlight the significance of the parameter~$f$ and clarify the necessary adjustments when processes lack knowledge of such a parameter.
We begin by presenting the Discovery algorithm.

\vspace{0.5em}
\noindent\textbf{Discovery algorithm.}
The Discovery algorithm illustrated in Algorithm~\ref{alg:discovery:known:f} enables any correct process~$i$ to expand the set of processes it knows with the aim of eventually receiving the PD of each correct process reachable from it. 
This algorithm provides only one task, $\mathtt{discovery}$.
When a process executes this task, it periodically asks the processes it knows to respond by sending the PDs they have received. 
% 
\begin{algorithm}[!t]
\caption{The Discovery algorithm -- process $i$.}
\label{alg:discovery:known:f}
\begin{algorithmic}[1]
\NoThen\NoDo
    \STATEx{\hspace{-1.67em}\textbf{task} $\mathtt{discovery}()$}
        \STATE{$\mathit{pds} \leftarrow \{ \langle i, \mathit{PD}_i \rangle_i \}$}\label{line:sign}
        \STATE{$\mathit{known} \leftarrow \mathit{PD}_i \cup \{i\}$}
        \STATE{$\mathit{received} \leftarrow \{i\}$}
        \STATE{\textbf{periodically} $\forall \ j \in \mathit{known}:$ \textbf{send} $\langle \textsc{GetPDs} \rangle$ \textbf{to} $j$}\label{line:get:pds}

    \vspace{0.5em}
    \STATEx{\hspace{-1.67em}\textbf{upon receiving} $\langle \textsc{GetPDs} \rangle$ \textbf{from} $j$}
    \STATE{\textbf{send} $\langle \textsc{PDs}, \mathit{pds} \rangle$ \textbf{to} $j$}

    \vspace{0.5em}
    \STATEx{\hspace{-1.67em}\textbf{upon receiving} $\langle \textsc{PDs}, \mathit{pds}_j \rangle$ \textbf{from} $j$}  
    \IF{$\langle j, \mathit{PD}_j\rangle_j \in \mathit{pds}_j$}
        \STATE{$\mathit{pds} \leftarrow \mathit{pds} \cup \mathit{pds}_j$}\label{line:start:update}
        \STATE{$\mathit{known} \leftarrow \mathit{known} \cup \{ k \in \mathit{PD}_* \ | \ \langle *, \mathit{PD}_*\rangle_* \in \mathit{pds}_j \}$}
        \STATE{$\mathit{received} \leftarrow \mathit{received} \cup \{ k \ | \ \langle k, *\rangle_* \in \mathit{pds}_j \}$}\label{line:end:update}
    \ENDIF
    \end{algorithmic}
\end{algorithm}
% 
Each process $i$ has the following three local sets:
\begin{itemize}
    \item $\mathit{pds}$ -- Process $i$ stores any received PD in this set, initialized with $\{\langle i, \mathit{PD}_i \rangle\}$.
    % 
    \item $\mathit{known}$ -- This set contains the processes that $i$ knows, initialized with $\mathit{PD}_i \cup \{i\}$.
    % 
    \item $\mathit{received}$ -- This set contains the set of processes that $i$ has received their PDs, initialized with $\{i\}$.
\end{itemize}

Periodically, each process~$i$ sends a $\langle \textsc{GetPDs} \rangle$ message to all processes it knows, requesting each of them to share its $\mathit{pds}$ (line~\ref{line:get:pds}).
Upon receiving a $\langle \textsc{GetPDs} \rangle$ request from process~$j$, process~$i$ responds by sending the PDs it knows, i.e., sending set $\mathit{pds}$ to $j$. 
When $i$ receives a message $\langle \textsc{PDs}, \mathit{pds}_j \rangle$ from process $j$, it updates its local sets using $\mathit{pds}_j$ (lines~\ref{line:start:update}-\ref{line:end:update}).
This algorithm satisfies the following two properties expressed as theorems.
\begin{theorem}\label{thm:discovery:sink}
    Consider a system with a knowledge connectivity graph $G_{\mathit{di}} \in \mathcal{G}_\mathit{di}$. 
    Assuming $V_{\mathit{sink}}$ comprises the sink members of $G_{\mathit{di}}$, by executing Algorithm~\ref{alg:discovery:known:f} in this system, every correct process eventually
    \begin{enumerate*}[label=(\alph*)]
        \item discovers all sink members, i.e., 
        $\forall \ i \in C: V_{\mathit{sink}} \cap C \subseteq \mathit{known}$, and
        % 
        \item receives the PDs of all correct sink members, i.e.,
        $\forall \ i \in C: V_{\mathit{sink}} \cap C \subseteq \mathit{received}$.\qed
    \end{enumerate*}
     
\end{theorem}
The proof of the aforementioned theorem, as well as other theorems presented throughout the paper, can be found in the full version of the paper~\cite{full_version}.
It is worth noting that, since correct processes sign their PDs (line~\ref{line:sign}), Byzantine processes cannot lie about the PD of a correct process, either by modifying the PD of a correct process or by creating a PD for a correct process.

\vspace{0.5em}
\noindent\textbf{Sink algorithm.}
Before delving into the Sink algorithm, we present a preliminary result about the sink component.
We begin by demonstrating the result for a particular case.
With this aim, consider the knowledge connectivity graph depicted in Fig.~\ref{fig:osr:example:possible} in which each process in set $V_{\mathit{safe}} = \{1,2,3\}$ knows Byzantine process~$4$.
In this graph, if process $4$ sends $V_{\mathit{safe}}$ as $\mathit{PD}_4$ to processes in $V_{\mathit{safe}}$, each process $i \in V_{\mathit{safe}}$ cannot make a distinction between this situation and the following situation: the system is composed of $4$ correct processes $1$, $2$, $3$, and $4$, and $\mathit{PD}_i=\{1,2,3,4\}\setminus\{i\}$ for each process $i\in \{1,2,3,4\}$. 
Note that each process in $V_{\mathit{safe}}$ identifies $\{1,2,3,4\}$ as the sink in the second situation; as these situations are indistinguishable for processes in $V_{\mathit{safe}}$, they must identify $\{1,2,3,4\}$ as the sink in the first situation as well.

The generalization of this particular case is presented in the theorem below.
This theorem indeed enables each correct process to identify the sink when a subset of sink members in the safe subgraph of $G_{\mathit{di}}$ initially know some Byzantine process(es).
It is essential to note that this theorem considers Byzantine processes; however, Theorem~\ref{thm:bft:cup} exclusively specifies the properties of the safe subgraph of $G_{\mathit{di}}$.

\begin{theorem}\label{thm:sink:alternative:def}
    Given a knowledge connectivity graph $G_{\mathit{di}}=(V_{\mathit{di}},E_{\mathit{di}})$ that belongs to $\mathcal{G}_{\mathit{di}}$, if a subset of processes $S$ satisfies the following properties, it contains all sink members:
    \begin{enumerate}[label=P\arabic*)]
        \item The strong connectivity of $S$ is greater than or equal to $f+1$, i.e., $\kappa(S) \geq f+1$.
        \item The number of node-disjoint paths from $S$ to any other subset of processes in $G_{\mathit{di}}$ is bounded by $f$, i.e.,
        $\forall \ T \subseteq  V_{\mathit{di}} \setminus S$ : $S \xRightarrow[]{\leq f} T$.\qed
    \end{enumerate}
\end{theorem}

We now provide an insight into the properties specified in the aforementioned theorem.
\begin{itemize}
    \item \textbf{Property P1}. 
    Since $G_\mathit{di} \in \mathcal{G}_{\mathit{di}}$, the subgraph that contains only correct sink members is $(f+1)$-strongly connected (according to Theorem~\ref{thm:bft:cup}).
    Besides, a Byzantine process~$i$ known by some correct sink member(s), like Byzantine process $4$ in Fig.~\ref{fig:osr:example:possible}, can be a member of the sink if it has at least $f+1$ node-disjoint paths to correct sink members, and correct sink members have at least $f+1$ node-disjoint paths to $i$.
    Consequently, the connectivity of the sink must be at least $f+1$.
    % 
    \item \textbf{Property P2}. 
    According to Theorem~\ref{thm:bft:cup}, no correct sink member has a link to a correct non-sink member.
    However, Byzantine sink members can have links to non-sink members.
    As there are at most $f$ Byzantine sink members, the number of node-disjoint paths from the sink to the outside of the sink is limited by $f$, which is presented by Property P2.
\end{itemize}

Taking into account the existence of Byzantine processes in the sink, the Sink algorithm (Algorithm~\ref{alg:sink:known:f}) enables each process $i$ to discover the sink members when the knowledge connectivity graph $G_{\mathit{di}} \in \mathcal{G}_\mathit{di}$.
%We are now ready to present the Sink algorithm.
%In a system with a knowledge connectivity graph $G_{\mathit{di}} \in \mathcal{G}_\mathit{di}$, the Sink algorithm (Algorithm~\ref{alg:sink:known:f}) enables each process $i$ to discover the sink members.
This algorithm provides only one function, $\mathtt{sink}$.
Using this function, each correct process continuously expands the set of processes it knows by executing the Discovery algorithm until it identifies the sink component.
It terminates the Sink algorithm by returning a set equal to $V_{\mathit{sink}}$ when there exists two sets $K$ and $R$ with conditions specified in line~\ref{line:sink:condition}.
These conditions are analogous to the properties specified in Theorem~\ref{thm:sink:alternative:def}.
It then returns $K \cup R$ as the discovered sink.
% Specifically, it waits until there exists a set $R \subseteq \mathit{received}$ such that $\kappa(R) \geq f+1$ and $R$ is maximal in the sense that there is no process $j$ for which $\kappa(R\cup \{j\})\geq f+1$.
% Process $i$ to ensure Property P2 and there is no subset of processes $T\subseteq \mathit{received}$ that 
% Once these conditions are satisfied, the algorithm returns $K\cup R$, indicating the identified sink component.

\begin{algorithm}[t!]
\caption{The Sink algorithm -- process $i$.}
\label{alg:sink:known:f}
\begin{algorithmic}[1]
\NoThen\NoDo
    
    \STATEx{\hspace{-1.67em}\textbf{function} $\mathtt{sink}()$}
    \STATE{\textbf{fork} $\mathtt{discovery}()$}

    \STATE{\textbf{wait until} $\exists \ R\subseteq \mathit{received}: \kappa(R) \geq f+1 \ \land$}
    \STATEx{$\boldsymbol{(} \exists \ K \subseteq \mathit{known}\setminus \mathit{received} : R \xRightarrow[]{> f} K \rightarrow |K| \leq f \boldsymbol{)}$}
    % \STATEx{$\boldsymbol{(} \nexists \ j \in \mathit{received} : \kappa(R\cup \{j\}) \geq f+1 \boldsymbol{)}$}
    \label{line:sink:condition}
    \STATE{\textbf{return} $K \cup R$}
    
\end{algorithmic}
\end{algorithm}

Using an example, we demonstrate why the Sink algorithm returns $K \cup R$ as the sink.
Consider the knowledge connectivity graph depicted in Fig.~\ref{fig:osr:example:possible}.
Suppose process $1$ executes the $\mathtt{sink}$ function, and consider the following scenario.
Process $2$ is slow, and process $4$ sends a set $P=\{1,2,3\}$ as its PD during the execution of $\mathtt{discovery}$.
When process $1$ receives $P$ and $\mathit{PD}_3$, the conditions specified in line~\ref{line:sink:condition} of Algorithm~\ref{alg:sink:known:f} are satisfied.
Therefore, $R=\{1,3,4\}$ and $K=\{2\}$.
As set $\{1,2,3,4\}$ is the sink, $K \cup R$ must be returned as the result.

The Sink algorithm satisfies the following properties expressed as theorems.
\begin{theorem}\label{thm:sink:termination}
    In a knowledge connectivity graph $G_{\mathit{di}} \in \mathcal{G}_{\mathit{di}}$, Algorithm~\ref{alg:sink:known:f} executed by any correct process eventually terminates.\qed
\end{theorem}
\begin{theorem}\label{thm:sink:sink}
    In a knowledge connectivity graph $G_{\mathit{di}} \in \mathcal{G}_{\mathit{di}}$, Algorithm~\ref{alg:sink:known:f} executed by any correct process returns all sink members.\qed
\end{theorem}
% In Appendix~\ref{appendix:sink}, we present the proofs of these theorems.

\vspace{0.5em}
\noindent\textbf{Solving consensus in the authenticated BFT-CUP model.}
Algorithm~\ref{alg:consensus} solves consensus in the authenticated BFT-CUP model.
This algorithm provides a $\mathtt{propose}$ function through which processes can propose a value and decide on a common value.
In this algorithm, each process $i$ first executes the Sink algorithm.
Upon the termination of the Sink algorithm, process $i$ acts based on whether it is a sink or a non-sink member.
If it is a sink member, it executes a traditional consensus protocol (e.g., PBFT~\cite{castro_1999}) with the sink members.
% Otherwise, it asks sink members to respond by sending the decided value and waits until receiving $f+1$ matching responses.
% Since the sink component contains at most $f$ Byzantine processes, there is at least one response sent by a correct sink member.
Otherwise, it asks sink members to respond by sending the decided value and waits until receiving the same value from $\ceil{(|S|+1)/2}$ distinct sink members, where $S$ comprises the sink members.
Since the sink component contains at least $2f+1$ correct processes while there are at most $f$ Byzantine processes in the sink, $\ceil{(|S|+1)/2}\geq f+1$.
This implies that there is at least one correct process among the responded processes.

\begin{algorithm}[t!]
\caption{The Consensus algorithm -- process $i$.}
\label{alg:consensus}
\begin{algorithmic}[1]
\NoThen\NoDo
    \STATEx{\hspace{-1.67em}\textbf{variables}}
    \STATE{$\mathit{val} \leftarrow \perp$}

    \vspace{0.5em}
    \STATEx{\hspace{-1.67em}\textbf{function} $\mathtt{propose}(v)$}
    \STATE{$S \leftarrow \mathtt{sink}()$}
    \IF{$i \in S$}
        \STATE{$\mathit{val} \leftarrow \mathtt{consensus}.\mathtt{propose}(S,v)$}
    \ELSE
        \STATE{$\forall \ j \in S: $ \textbf{send} $\langle \textsc{GetDecidedVal} \rangle$ \textbf{to} $j$}
        \STATE{\textbf{wait until receiving the same} $\langle \textsc{DecidedVal}, \mathit{val} \rangle$}
        \STATEx{\qquad \textbf{from} $\ceil{(|S|+1)/2}$ distinct processes in $S$}
    \ENDIF
    \STATE{\textbf{return} $\mathit{val}$}

    \vspace{0.5em}
    \STATEx{\hspace{-1.67em}\textbf{upon receiving} $\langle \textsc{GetDecidedVal} \rangle$ \textbf{from} $j$}
    \STATE{\textbf{wait until} $\mathit{val} \neq \perp$}
    \STATE{\textbf{send} $\langle \textsc{DecidedVal}, \mathit{val} \rangle$ \textbf{to} $j$}
\end{algorithmic}
\end{algorithm}

\begin{theorem}
    Algorithm~\ref{alg:consensus} solves consensus in the authenticated BFT-CUP model.\qed
\end{theorem}

\subsection{The Fault Threshold's Role in the BFT-CUP Model}
In the three algorithms presented to solve consensus in the authenticated BFT-CUP model, the only place where the fault threshold is used is in the Sink algorithm (Algorithm~\ref{alg:sink:known:f}).
In that algorithm, each process requires knowing the value of $f$ in order to identify the sink and terminate the algorithm.
Consequently, the lack of access to $f$ may lead to the following scenarios:
\begin{enumerate*}[label=(\alph*)]
    \item the Sink algorithm does not terminate,
    \item multiple subsets of the sink might declare themselves as the sink, or
    \item a subset of non-sink members might declare themselves as the sink.
\end{enumerate*}
As processes require to discover the sink to solve consensus, the Termination property of consensus is violated if the first scenario happens.
If the second and third scenarios happen, the Agreement property of consensus can be violated as each sink can solve consensus independently of other processes.

\section{Problem Specification and an Impossibility Result}\label{sec:problem:specification}
Solving consensus in the BFT-CUP model requires that the information provided by the participant detectors of all processes collectively form a knowledge connectivity graph that satisfies the requirements of the BFT-CUP model.
Furthermore, it requires that each process~$i$ knows $\mathit{PD}_i$ and is provided with the value of $f$.
This paper intends to extend the BFT-CUP model to enable processes to solve consensus without knowing $f$.
We achieve it by assuming each process $i$ takes only $\mathit{PD}_i$ as input, and our goal is to find the necessary and sufficient knowledge connectivity requirements for solving consensus in this setting.

The initial step for finding such requirements involves addressing the following question:
\emph{is having a knowledge connectivity graph that satisfies the requirements of the BFT-CUP model sufficient to solve consensus when the fault threshold is unknown?} 
That is, can processes solve consensus when each process $i$ initially has access to its participant detector $\mathit{PD}_i$, the processes' participant detectors collectively form a knowledge connectivity graph $G_{\mathit{di}} \in \mathcal{G}_{\mathit{di}}$, and no process knows the value of $f$?
Notice the system still has a fault threshold as required to define $G_{\mathit{di}}$, but it is unknown.
We negatively answer the above question using the indistinguishability technique (e.g., used in ~\cite{flp, waitFree}), the sketch of which follows. 

\subsection{An Impossibility Result}
Consider two separate distributed systems $A$ and $B$ composed of disjoint and non-empty sets of processes $\Pi_A$ and $\Pi_B$, respectively. 
Assume that the knowledge connectivity graph formed by members of each system belongs to $\mathcal{G}_{\mathit{di}}$.
If each system intends to solve consensus, it can end up with a distinct decided value, as the processes of these systems are disjoint.
Next, suppose we build a distributed system $\mathit{AB}$ composed of $\Pi_A \cup \Pi_B$ by adding links between them so that the knowledge connectivity graph formed by members of $\mathit{AB}$ belongs also to $\mathcal{G}_{\mathit{di}}$.
We argue that the execution of consensus in $A$ (resp. $B$) is indistinguishable from the execution of consensus in $\mathit{AB}$ to the members of $\Pi_A$ (resp. $\Pi_B$).
Consequently, if $\mathit{AB}$ intends to solve consensus, the decided value by members of $\Pi_A$ may differ from that of members of $\Pi_B$, resulting in an Agreement violation.
The following theorem states the impossibility.

\begin{figure}[t!]
\centering
\begin{subfigure}[t]{0.22\textwidth}
    \centering
    \includegraphics[scale=0.8]{figures/impossibility-1.pdf}
    \caption{System A: a 2-OSR PD in which only process $4$ is faulty.}
    \label{fig:imp:a}
\end{subfigure}%
\hfill
\begin{subfigure}[t]{0.22\textwidth}
    \centering
    \includegraphics[scale=0.8]{figures/impossibility-2.pdf}
    \caption{System B: a 2-OSR PD in which only process $5$ is faulty.}
    \label{fig:imp:b}
\end{subfigure}
\\
\begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[scale=0.8]{figures/impossibility-3.pdf}
    \caption{System AB: a 1-OSR PD in which all processes are correct.}
    \label{fig:imp:c}
\end{subfigure}

\caption{Processes in $\{1,2,3\}$ cannot distinguish between case \ref{fig:imp:a} (if process $4$ remains silent) and case \ref{fig:imp:c} (if process $4$ is slow). 
Likewise, Processes in $\{6,7,8\}$ cannot distinguish cases \ref{fig:imp:b} and \ref{fig:imp:c}.}
\label{fig:imp}
\end{figure}

\begin{theorem}
    A knowledge connectivity graph that belongs to $\mathcal{G}_\mathit{di}$ is insufficient to solve consensus when the fault threshold is unknown.\qed
\end{theorem}
\begin{proof}
    We establish the theorem for a weaker failure model, specifically crash faults, by assuming that a process fails by crashing. 
    Given that any impossibility result derived for a weaker model holds for a stronger model, an impossibility result drawn for crash faults is also valid for Byzantine faults.
    
    For the sake of contradiction, assume that there is a protocol $\mathcal{A}$ by which processes can solve consensus when the knowledge connectivity graph of the system belongs to $\mathcal{G}_\mathit{di}$, but no process knows the value of the fault threshold.
    We present three cases, each with a corresponding knowledge connectivity graph. 
    It is straightforward to validate that each knowledge connectivity graph belongs to $\mathcal{G}_\mathit{di}$.
    \begin{enumerate}[label=\Roman*)]
        \item Consider a distributed system $A$ composed of a set of processes $\Pi_A=\{1,2,3,4\}$ with the knowledge connectivity graph depicted in Fig.~\ref{fig:imp:a}.
        Except for process $4$, other processes are correct.    
        Assume that the initial value of every process is $v$.
        Additionally, assume that the GST occurs at most by time $\Delta_A$ in this system (in accordance with the definition of partial synchrony, making such an assumption is possible).
        By assumption, processes $1,2,$ and $3$ must be able to solve consensus using $\mathcal{A}$.
        Let $E_A$ be an execution of $\mathcal{A}$ with duration $t_A$, resulting in deciding $v$ because of the Validity property of consensus.

        \item Similar to the previous case, consider a distributed system $B$ composed of a set of processes $\Pi_B=\{5,6,7,8\}$ with the knowledge connectivity graph depicted in Fig.~\ref{fig:imp:b}.
        Except for process $5$, other processes are correct.    
        Assume that the initial value of every process is $u$.
        Additionally, assume that the GST occurs at most by time $\Delta_B$ in this system.
        By assumption, processes $6,7,$ and $8$ must be able to solve consensus using $\mathcal{A}$.
        Let $E_B$ be an execution of $\mathcal{A}$ with duration $t_B$, resulting in deciding $u$ because of the Validity property of consensus.   

        \item Consider a distributed system $\mathit{AB}$ composed of eight processes $\Pi_A\cup \Pi_B = \{1,2,\dots, 8\}$ with the knowledge connectivity graph depicted in Fig.~\ref{fig:imp:c}.
        Assume that all processes are correct and the initial value of each member of $\Pi_A$ (resp. $\Pi_B$) is $v$ (resp. $u$). 
        The communication delays between any two members of $\{1,2,3\}$ (resp. $\{6,7,8\}$) is at most $\Delta_A$ (resp. $\Delta_B$); however, the communication delay between any other two processes is greater than $\mathtt{max}\{\Delta_{A}, \Delta_{B}, t_{A}, t_{B}\}$.
        Note that processes $1,2,$ and $3$ cannot distinguish cases I and III, so they must decide $v$.
        Likewise, processes $6,7,$ and $8$ cannot distinguish cases II and III, so they must decide $u$.
        Thus, the Agreement property is violated.
    \end{enumerate}

    The violation of the Agreement property of consensus in the third case implies a contradiction. 
    Consequently, our assumption that states there is a protocol by which processes can solve consensus when the fault threshold is unknown and the knowledge connectivity graph of the system belongs to $\mathcal{G}_\mathit{di}$ is incorrect.
    It follows that a knowledge connectivity graph that belongs to $\mathcal{G}_\mathit{di}$ is insufficient to solve consensus when the fault threshold is unknown, completing the proof.
\end{proof}

The impossibility result described above occurs because there are some executions where no process in $\{1,2,3\}$ can discover a process in $\{6,7,8\}$ and vice versa.
Indeed, two subsets of the sink can declare themselves as the sink.
Similarly, a subset of non-sink members might declare themselves as the sink.
For example, in Fig.~\ref{fig:imp:ns:b}, processes in $\{2,3,4,6\}$ that are non-sink members can declare themselves as the sink.
If that happens, the Agreement property of consensus can be violated as each sink can solve consensus independently of other processes.
In the subsequent section, we show how to enrich a knowledge connectivity graph that satisfies the requirements of the BFT-CUP model by adding extra edges so that consensus can be solved on the new graph without having access to $f$. 

\begin{figure}[t!]
\centering
\begin{subfigure}[t]{0.26\textwidth}
    \centering
    \includegraphics[scale=0.8]{figures/impossibility-1-ns-full.pdf}
    \caption{System A: a 2-OSR PD in which only process $1$ is faulty.}
    \label{fig:imp:ns:b}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.2\textwidth}
    \centering
    \includegraphics[scale=0.8]{figures/impossibility-1-ns.pdf}
    \caption{System B: a 3-OSR PD in which processes $5$ and $7$ are faulty.}
    \label{fig:imp:ns:a}
\end{subfigure}%

\caption{Processes in $\{2,3,4,6\}$ cannot distinguish between case \ref{fig:imp:ns:a} (if processes $5$ and $7$ remain silent) and case \ref{fig:imp:ns:b} (if process $1$ behaves like correct processes but processes $5$ and $7$ are slow).}
\label{fig:imp:non:sink}
\end{figure}
    
\section{The BFT-CUPFT Model}\label{sec:extended:bft:cup}
The primary challenge in solving consensus in the BFT-CUPFT model, when the initial knowledge of processes collectively forms a knowledge connectivity graph that belongs to $\mathcal{G}_{\mathit{di}}$, lies in the possibility of existing multiple subsets of processes, each identifying itself as a sink component.
Since processes within a sink can independently execute an instance of consensus without coordination with processes outside of that sink, the Agreement property of consensus may be compromised in the presence of multiple sinks.
To address this issue, it is crucial to prevent the emergence of multiple subsets of processes that mistakenly identify themselves as sinks.
This objective is accomplished in this section by adding extra edges to the knowledge connectivity graphs belonging to $\mathcal{G}_{\mathit{di}}$, i.e., increasing the required knowledge of processes, resulting in the introduction of a new type of knowledge connectivity graphs.
We begin by presenting an insight into the properties of such graphs.

\vspace{0.5em}
\noindent\textbf{Insight into the new type of knowledge connectivity graphs.}
In order to define the new knowledge connectivity graphs, we first need to understand when a subset of processes mistakenly declares themselves as a sink.
Recall that Theorem~\ref{thm:sink:alternative:def} states a set of processes $S \subseteq \Pi$ is a sink if and only if the following properties are satisfied:
$\kappa(S) \geq f+1$, and
$\forall \ T \subseteq \Pi \setminus S$, $S \xRightarrow[]{\leq f} T$. 
When processes lack knowledge of the value of $f$, consider a subset of processes $P$ with the same aforementioned properties except that, instead of $f$, there is a non-negative integer $y$ for which the properties hold.
Specifically, $P$ satisfies the following properties: 
$\kappa(P) \geq y+1$, and
$\forall \ T \subseteq \Pi \setminus P$, $P \xRightarrow[]{\leq y} T$. 
Since members of $P$ do not know the value of $f$, they consider themselves a sink (like processes in $\{1,2,3\}$ in the graph depicted in Fig.~\ref{fig:imp:c}).
% , which is formally proved in the following theorem.

% \begin{theorem}
% Consider there is a non a subset of processes $P$ that satisfies the following properties: 
% $\kappa(S) \geq y+1$, and
% $\forall \ T \subseteq \Pi \setminus S$, $S \xRightarrow[]{\leq y} T$.
% Members of $P$ declare themselves as a sink.
% \end{theorem}

We now define a new type of knowledge connectivity graphs in order to reduce the number of subsets of processes that consider themselves as sinks into a single subset.
We accomplish this by establishing outgoing links from a subset of processes $P$, which mistakenly identifies itself as a sink. 
This addition of links serves to augment the number of node-disjoint paths from $P$ to processes not belonging to $P$, ensuring that the second property mentioned above does not hold for $P$.
Accordingly, $P$ cannot declare itself as a sink.
% Also, the new links increase the knowledge of processes in $P$.
We call the unique subset of processes that consider themselves as a sink by \textit{core}.

Fig.~\ref{fig:rich:k:osr} shows an example of how processes in $\{5,6,7,8\}$ were prevented from mistakenly identifying themselves as a sink when $5$ is slow by adding an extra link from process $6$ to $3$.
In the resulting graph with an extra link, processes in $\{5,6,7,8\}$ cannot identify themselves as a sink, as they discover the existence of processes $1$, $2$, $3$, and $4$ even if process $5$ is slow.
Hence, the mentioned properties do not hold for multiple disjoint subsets of processes in that graph, solving the issue.

\begin{figure}[t!]
\centering
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[scale=0.8]{figures/rich-k-osr.pdf}
    \caption{In this knowledge connectivity graph, the sink component differs from the core component.}
    \label{fig:rich:k:osr}
\end{subfigure}
\\
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[scale=0.8]{figures/rich-k-osr-2.pdf}
    \caption{In this knowledge connectivity graph, the sink component is the same as the core component.}
    \label{fig:rich:k:osr:2}
\end{subfigure}

\caption{Two knowledge connectivity graphs that satisfy the requirements of the BFT-CUPFT model.}
\label{fig:rich:k:osr:all}
\end{figure}

\vspace{0.5em}
\noindent\textbf{New type of knowledge connectivity graphs.}
In order the specify the properties of the knowledge connective graphs in which we can solve consensus without knowing the fault threshold, we first extend the definition of $k$-OSR PD.

\begin{definition}[Extended $k$-OSR PD]\label{def:eosr}
A knowledge connectivity graph $G_{\mathit{di}}=(V_{\mathit{di}},E_{\mathit{di}})$ belongs to extended $k$-OSR PD if it satisfies the following properties:
\begin{itemize}
    \item it belongs to $k$-OSR PD; hence, the graph contains exactly one sink component $G_{\mathit{sink}}=(V_{\mathit{sink}},E_{\mathit{sink}})$, and
    \item there is a non-negative integer $y$ such that exactly one set of processes $P \subseteq V_{\mathit{sink}}$, namely the \textit{core}, satisfies the following two conditions:
    \begin{itemize}
        \item $\kappa(P) \geq y+1$, and
        \item $\forall \ T \subseteq \Pi \setminus P$, $P \xRightarrow[]{\leq y} T$.\qed
    \end{itemize}
\end{itemize}    
\end{definition}
The knowledge connectivity graph defined using the extended $k$-OSR PD enables processes to solve consensus without having knowledge about the fault threshold.
The following theorem formalized this.
\begin{theorem}\label{thm:bft:cupft}
The following three properties must be satisfied to ensure solving consensus in the BFT-CUPFT model:
\begin{itemize}
\item $G_{\mathit{safe}}$ belongs to the $(f+1)$-OSR PD,
\item the sink component of $G_{\mathit{safe}}$ must contain at least $2f+1$ processes,
\item the core component of $G_{\mathit{safe}}$ must contain at least $2f+1$ processes.\qed
\end{itemize}
\end{theorem}
If a knowledge connectivity graph meets the properties of Theorem~\ref{thm:bft:cupft}, we say it satisfies the requirements of the BFT-CUPFT model.
The graphs depicted in Fig.~\ref{fig:rich:k:osr:all} are examples of knowledge connectivity graphs that satisfy the requirements of the BFT-CUPFT.

\section{Consensus in the BFT-CUPFT Model}\label{sec:consensus:extended:bft:cup}
This section presents a protocol that solves consensus in the BFT-CUPFT model. 
Recall that in Section~\ref{sec:revisiting:bft:cup}, we presented three algorithms~-- Discovery, Sink, and Consensus~-- to solve consensus in the authenticated BFT-CUP model. 
Since processes can execute the Discovery and Consensus algorithms without knowing the fault threshold, we can employ them in scenarios where the fault threshold is unknown.
Since there is only one core in a knowledge connectivity graph that satisfies the requirements of the BFT-CUPFT model, we design an algorithm called Core that allows processes to discover the core component.
We then use the Core algorithm instead of the Sink algorithm in the Consensus algorithm for solving consensus in the BFT-CUPFT model.

\vspace{0.5em}
\noindent\textbf{The Core algorithm in the BFT-CUPFT model.}
The objective of the Core algorithm in the BFT-CUPFT model is to allow each process $i$ to discover the core members.
In further detail, each process expands the set of processes it knows by executing the Discovery algorithm.
It continues executing the $\mathtt{discovery}$ task until it identifies the core component.
Afterward, any correct process $i$ terminates by returning a set that contains all core members.
The following theorem determines how a process can identify whether a set of processes is the core.
\begin{theorem}\label{thm:sink:alternative:def:wf}
In a knowledge connectivity graph that satisfies the requirements of the BFT-CUPFT model in which a set $P$ comprises the core members, there exists exactly one non-negative integer $y$ for which the following properties are satisfied:
    \begin{itemize}
        \item $\kappa(P) \geq y+1$, and
        \item  $\forall \ T \subseteq \Pi \setminus P$, $P \xRightarrow[]{\leq y} T$.\qed
    \end{itemize}
\end{theorem}
The Core algorithm is shown in Algorithm~\ref{alg:sink}.
This algorithm provides only one function, $\mathtt{core}$.
Upon initiation, the algorithm forks the $\mathtt{discovery}$ task, allowing concurrent execution of the Discovery algorithm. 
Process $i$ waits until the properties specified in Theorem~\ref{thm:sink:alternative:def:wf} are satisfied for a subset of processes. 
Specifically, it waits until there exists two sets $K$ and $R$ with the conditions specified in line~\ref{line:condition:core}.
Once these conditions are satisfied, the algorithm returns $K\cup R$, indicating the identified core component.
The Core algorithm satisfies the following properties expressed as theorems.
\begin{theorem}\label{thm:sink:termination:wf}
    In a knowledge connectivity graph that satisfies the requirements of the BFT-CUPFT model, 
    Algorithm~\ref{alg:sink} executed by any correct process eventually terminates.\qed
\end{theorem}
\begin{theorem}\label{thm:sink:sink:wf}
    In a knowledge connectivity graph that satisfies the requirements of the BFT-CUPFT model, 
    Algorithm~\ref{alg:sink} executed by any correct process returns all core members.\qed
\end{theorem}
Finally, in order to solve consensus in the BFT-CUPFT model, in the Consensus algorithm outlined in Algorithm~\ref{alg:consensus}, we use the Core algorithm instead of the Sink algorithm.
The following theorem states that the requirements presented in Theorem~\ref{thm:bft:cupft} are sufficient to solve consensus in the BFT-CUPFT model.
\begin{theorem}
    In a knowledge connectivity graph that satisfies the requirements of the BFT-CUPFT model, 
    processes can solve consensus by executing the Core algorithm instead of the Sink algorithm in Algorithm~\ref{alg:consensus}.\qed
\end{theorem}

\begin{algorithm}[t!]
\caption{The Core algorithm in the BFT-CUPFT model -- process $i$.}
% \fontsize{9.5}{12}
\label{alg:sink}
\begin{algorithmic}[1]
\NoThen
\NoDo

\STATEx{\hspace{-1.67em}\textbf{function} $\mathtt{core}()$}
    \STATE{\textbf{fork} $\mathtt{discovery}()$}

    \STATE{\textbf{wait until} $\exists \ y \geq 0, \exists \ R\subseteq \mathit{received}: \kappa(R) \geq y+1 \ \land$}
    \STATEx{$\boldsymbol{(} \exists \ K \subseteq \mathit{known}\setminus \mathit{received} : R \xRightarrow[]{> y} K \rightarrow |K| \leq y \boldsymbol{)}$}\label{line:condition:core}
    
    % \STATE{\textbf{wait until} $\exists \ y \geq 0, \exists \ R\subseteq \mathit{received}: \kappa(R) \geq y+1 \ \land$}
    % \STATEx{$\boldsymbol{(} \exists \ K \subseteq \mathit{known}\setminus \mathit{received} :  R \xRightarrow[]{> y} K \rightarrow |K| \leq y \boldsymbol{)} \ \land$}
    % \STATEx{$\boldsymbol{(} \nexists \ j \in \mathit{received} : \kappa(R\cup \{j\}) \geq y+1 \boldsymbol{)}$}\label{line:condition:core}
    \STATE{\textbf{return} $K \cup R$}

\end{algorithmic}
\end{algorithm}

\section{Related Work}\label{sec:related:work}
\noindent\textbf{Consensus with Unknown Participants.}
The evolution of the Consensus with Unknown Participants (CUP) problem has involved a series of advancements to accommodate diverse system models. 
Initially, Cavin et al.~\cite{cavin_2004} defined the problem for failure-free asynchronous systems, introducing a participant detector abstraction to provide initial information about system membership. 
The information collectively forms a knowledge connectivity graph, and that work establishes the necessary and sufficient properties that knowledge connectivity graphs must satisfy to solve the CUP problem. 
Subsequently, CUP was addressed in~\cite{cavin_2005} for crash-prone systems using the Perfect ($\mathcal{P}$) failure detector \cite{chandra_1996}. 
As implementing $\mathcal{P}$ requires synchrony, Greve and Tixeuil~\cite{greve_2007} relaxed the assumption to partial synchrony~\cite{dwork_1988} by augmenting the minimum required knowledge, specifically by increasing connections in the knowledge connectivity graph. 
This augmentation is demonstrated to be the minimum to tolerate crash failures without imposing synchrony requirements. 
The latest milestone extended CUP to tolerate Byzantine failures, introducing the BFT-CUP protocol~\cite{alchieri_2008, alchieri_2016}.

\vspace{0.5em}
\noindent\textbf{Consensus in directed graphs.}
Somewhat similar to the CUP model, several studies explore consensus in directed graphs, e.g.,~\cite{biely_2012,vaidya_2012,biely_2018,tseng_2015}.
Nevertheless, these investigations focus on determining the properties of the underlying communication graph to achieve consensus under diverse assumptions. 
For instance, Tseng and Vaidya~\cite{tseng_2015} established the minimal conditions of the underlying communication graph, where a participant $i$ can transmit messages to participant $j$ if a directed edge from $i$ to $j$ exists in the graph; otherwise, $i$ cannot send messages to $j$. 
Typically, these studies assume that the set of participants and the underlying communication graph are known to all participants. 
However, in the CUP model, the communication graph is complete, and the objective is to determine the necessary and sufficient initial knowledge about other participants required to solve consensus without knowing the system's membership.

\vspace{0.5em}
\noindent\textbf{Consensus on heterogeneous quorum systems.}
The exploration of protocols designed for systems where participants can have different trust assumptions, i.e., each participant can trust a subset of participants, originated in~\cite{damgard_2007}. 
Ripple~\cite{schawartz_2014,chase_2018} attempted to leverage this approach to address consensus in the permissionless setting, aiming to establish an efficient blockchain infrastructure. However, the achievement of this goal faced challenges leading to safety and liveness violations~\cite{amores_2020}. In contrast, Stellar~\cite{mazieres_2015,lokhava_2019}, based on the Federated Byzantine Quorum System (FBQS) formally studied later in~\cite{garcia_2018}, successfully achieved this objective.
In this approach, a network of trust emerges from the partial view declared by each participant. Consensus in this network is ensured if it adheres to the \emph{intact set} property, stipulating that all correct participants must form a quorum, and any two quorums formed by correct participants must intersect.
However, a recent comparison showed that the CUP model's initial knowledge is sufficient to solve consensus, even when processes know the fault threshold, compared with the Stellar model~\cite{vassantlal_2023}.

The connection between FBQS and dissemination Byzantine quorum systems~\cite{malkhi_1998} was established in~\cite{garcia_2018} and~\cite{garcia_2019}, illustrating the construction of a dissemination Byzantine quorum system corresponding to an FBQS. Subsequent work by Losa et al.~\cite{losa_2019} generalized FBQS to Personal Byzantine Quorum System (PBQS), demonstrating that consensus with weaker properties than the intact set is achievable through a \emph{consensus cluster}. Notably, forming a quorum by all correct participants is not mandatory within the consensus cluster.

Cachin and Tackmann~\cite{cachin_2019} extended Byzantine Quorum Systems (BQS)~\cite{malkhi_1998} from the symmetric trust model to the asymmetric model, facilitating a comparison between PBQS and the classical BQS model. Recently, Cachin et al. extended the asymmetric trust model, allowing each participant to make assumptions about the failures of participants it knows and, through transitivity, about failures of participants indirectly known by it~\cite{cachin_2022}.
Li et al.~\cite{li2023quorum} recently introduced heterogeneous quorum systems similar to PBQSs and demonstrated that the two properties~-- quorum intersection and availability~-- are necessary but insufficient to solve consensus.
They introduced the notion of quorum subsumption and established that the three conditions together are sufficient.

This line of research diverges from the CUP model in the following aspects. 
While these studies presume each process possesses a local fault threshold, the CUP model operates under the assumption of a global fault threshold. 
Furthermore, these studies identify the properties of quorums in order to solve consensus, whereas the CUP model outlines the requirements for knowledge connectivity graphs.

% \vspace{1em}
% \noindent\textbf{Consensus with unreliable channels.}

\vspace{0.5em}
\noindent\textbf{Sleepy model.}
The CUP model addresses consensus in partially synchronous systems, accommodating correct or faulty participants. However, this model assumes that correct members remain actively engaged throughout the entire execution, a condition that may be impractical in real-world scenarios.
In contrast, the sleepy model~\cite{momose_2022,pass_2017} introduces a different perspective. In this model, participants in a synchronous system are categorized as either awake or asleep, with awake participants capable of being either faulty or correct. The system's fault tolerance dynamically adjusts as participants transition between awake and asleep states. Crucially, consensus can be achieved if the majority of awake participants are correct at any given time. Moreover, unlike CUP, all participants in this model have knowledge of the system's membership.

\vspace{0.5em}
\noindent\textbf{Consensus using broadcast medium.}
Khanchandani and Wattenhofer~\cite{khanchandani_2021} established the impossibility of solving consensus in non-synchronous systems where participants and the fault threshold are unknown. In their system, \textit{no process initially possesses knowledge about other processes}, and each process utilizes a broadcast medium for communication. Recall that our primary goal in this paper is to solve consensus in partially synchronous systems, where each process lacks information about the system's membership and the fault threshold.
Accordingly, at first glance, our goal might appear contradictory to that impossibility result.
However, each process has knowledge about the existence of a subset of processes in our model (BFT-CUPFT), which is sufficient to discover the core component.
Recall that all processes discover the same core. 
The correct processes within the core can solve consensus and inform other processes about the decided value, resulting in solving consensus by all correct processes.
Hence, that impossibility result does not apply to our work.

\section{Conclusion}\label{sec:conclusion}
We addressed the critical challenge of solving Byzantine fault tolerant consensus in partially synchronous systems where each participant joins the network by having only partial knowledge about the existence of other participants and without explicit information about the fault threshold. 
We demonstrated that the key challenge arises from the possibility of having multiple disjoint subsets of processes, each solving a distinct instance of consensus, thereby violating the Agreement property of consensus. 
In order to mitigate this issue, we specified the necessary and sufficient knowledge connectivity requirements that must be satisfied to allow solving consensus in such settings.
% As done in the past to relax the setting in which CUP solves consensus, our solution to solve consensus without having explicit information about the fault threshold is to augment the knowledge connectivity graph with more connections.

\bibliographystyle{IEEEtran}
\bibliography{ref}

% \clearpage
% \section{Appendix}
% \subsection{The Proof Related to \texttt{verifyPD}}\label{appendix:verify:pd}
% \begin{proof}[Proof of Theorem~\ref{thm:verify:pd}] 
%     The following two properties must be satisfied by a knowledge connectivity graph $G_{\mathit{di}} = (V_{\mathit{di}},E_{\mathit{di}})$ to ensure solving consensus in the BFT-CUP model due to Theorem~\ref{thm:bft:cup}: 
%     \begin{enumerate*}[label=(\Roman*)]
%         \item the induced subgraph $G_{\mathit{safe}}$ belongs to the $(f+1)$-OSR PD, and 
%         \item the sink component of $G_{\mathit{safe}}$ must contain at least $2f+1$ processes.
%     \end{enumerate*}
%     In order to prove the theorem, we show that these properties must be satisfied even if no process can add new processes to the set received from its PD.
%     We initiate by focusing on Property I.

%     \vspace{0.5em}
%     \noindent\textbf{Property I.} 
%     Recall that $G_{\mathit{safe}}$ belongs to the $(f+1)$-OSR PD if it satisfies the following properties:
%     \begin{enumerate*}[label=(\roman*)]
%         \item the undirected graph $G$ obtained from $G_{\mathit{safe}}$ is connected,
%         \item the directed acyclic graph obtained by reducing $G_{\mathit{safe}}$ to its strongly connected components has exactly one sink, namely $G_\mathit{sink}=(V_\mathit{sink}, E_\mathit{sink})$,
%         \item the sink component $G_\mathit{sink}$ is $(f+1)$-strongly connected, and
%         \item there are at least $f+1$ node-disjoint paths from any process $i \notin V_\mathit{sink}$ to any process $j \in V_\mathit{sink}$.
%     \end{enumerate*}

%     \vspace{0.5em}
%     \noindent\textbf{Property i and Property ii.} 
%     Note that if $G$ is not connected, each component in $G$ can decide a distinct value, resulting in an Agreement violation.
%     Likewise, when there are multiple sinks, each sink can decide a distinct value.
%     Consequently, the fact that processes cannot provide false information about the sets received from their PDs has no effect on Property i and Property ii.

%     \vspace{0.5em}
%     \noindent\textbf{Property iii.} 
%     Regarding the connectivity of the sink component, for the sake of contradiction, assume the sink component of $G_{\mathit{safe}}$ does not need to be $(f+1)$-strongly connected; hence, consensus can be solved if it is $k$-strongly connected, where $k\leq f$.
%     Without loss of generality, assume $k=f$.
%     Consider the knowledge connectivity graph in Fig.~\ref{fig:sink:a} in which there is one Byzantine process, and its induced subgraph $G_{\mathit{safe}}$ is $1$-strongly connected. 
%     Due to our assumption, processes in this graph can solve consensus.
    
%     Note that processes $2$ and $3$ cannot make a distinction between the following two situations: 
%     (1) process $1$ is fast and Byzantine but process $4$ is slow and correct, and
%     (2) process $1$ is correct, but process $4$ is Byzantine and stays silent, and there are four processes in the system like the graph depicted in Fig.~\ref{fig:sink:b}.
%     Therefore, during solving consensus in graph Fig.~\ref{fig:sink:a}, if processes $2$ and $3$ receive messages from process $1$ before hearing from process $4$, they should not wait to receive a message from process $4$.
%     Assume the proposed value by processes $2$ and $3$ is $x$.
%     Consequently, they can decide on $x$.

%     Likewise, processes $5$ and $6$ cannot make a distinction between the following two situations: 
%     (1) process $1$ is fast and Byzantine but process $4$ is slow and correct, and
%     (2) process $1$ is correct, but process $4$ is Byzantine and stays silent, and there are four processes in the system like the graph depicted in Fig.~\ref{fig:sink:c}.
%     Therefore, during solving consensus in graph Fig.~\ref{fig:sink:a}, if processes $5$ and $6$ receive messages from process $1$ before hearing from process $4$, they should not wait to receive a message from process $4$.
%     Assume the proposed value by processes $5$ and $6$ is $y\neq x$.
%     Consequently, they can decide on $y$.
%     Since there is an Agreement violation, there is a contradiction, which means our assumption was incorrect.
%     Therefore, the fact that processes cannot provide false information about the sets received from their PDs has no effect on Property iii.

%     \begin{figure}[t!]
%         \centering
%         \begin{subfigure}[t]{0.22\textwidth}
%             \centering
%             \includegraphics[scale=0.8]{figures/sink-a.pdf}
%             \caption{A $1$-OSR PD in which process $1$ is Byzantine, and others are correct.}
%             \label{fig:sink:a}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[t]{0.22\textwidth}
%             \centering
%             \includegraphics[scale=0.8]{figures/sink-b.pdf}
%             \caption{A $1$-OSR PD in which process $4$ is Byzantine, and others are correct.}
%             \label{fig:sink:b}
%         \end{subfigure}%
%         \\
%         \begin{subfigure}[t]{0.22\textwidth}
%             \centering
%             \includegraphics[scale=0.8]{figures/sink-c.pdf}
%             \caption{A $1$-OSR PD in which process $4$ is Byzantine, and others are correct.}
%             \label{fig:sink:c}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[t]{0.22\textwidth}
%             \centering
%             \includegraphics[scale=0.8]{figures/sink-d.pdf}
%             \caption{A $1$-OSR PD in which process $4$ is Byzantine, and others are correct.}
%             \label{fig:sink:d}
%         \end{subfigure}
%         \caption{Four knowledge connectivity graphs used in the proof of Theorem~\ref{thm:verify:pd}.}
%         \label{fig:sink}
%     \end{figure}

%     \vspace{0.5em}
%     \noindent\textbf{Property iv.} 
%     Regarding the number of disjoint paths from a correct non-sink member to a correct sink member, for the sake of contradiction, assume $k$ node disjoint paths in $G_{\mathit{safe}}$ are required to solve consensus, where $k\leq f$.
%     Without loss of generality, assume $k=f$.
%     Consider the knowledge connectivity graph in Fig.~\ref{fig:sink:d} in which there is one Byzantine process, and its induced subgraph $G_{\mathit{safe}}$ is $1$-strongly connected. 
%     Due to our assumption, processes in this graph can solve consensus.
    
%     Note that processes $2$ and $3$ cannot make a distinction between the following two situations: 
%     (1)~process~$1$ is fast and Byzantine, but process $4$ is slow and correct, and
%     (2)~process~$1$ is correct, but process $4$ is Byzantine and stays silent, and there are four processes in the system like the graph depicted in Fig.~\ref{fig:sink:b}.
%     Therefore, during solving consensus in graph Fig.~\ref{fig:sink:d}, if processes $2$ and $3$ receive messages from process $1$ before hearing from process $4$, they should not wait to receive a message from process $4$.
%     Assume the proposed value by processes $2$ and $3$ is $x$.
%     Consequently, they can decide on $x$.

%     As processes within $\{5,6,7\}$ form the sink component, they can decide on a value independent of non-sink members. 
%     Assume the proposed value by processes $5$, $6$, and $7$ is $y\neq x$.
%     Consequently, they can decide on $y$.
%     Since there is an Agreement violation, there is a contradiction.
%     Therefore, the fact that processes cannot provide false information about the sets received from their PDs has no effect on Property iv.

%     \vspace{0.5em}
%     \noindent\textbf{Property II.} 
%     Assume all processes within $V_{\mathit{di}}$ are sink members.
%     Besides, assume each process initially knows all other processes, i.e., $\forall \ i \in \Pi : \mathit{PD}_i = \Pi\setminus \{i\}$.
%     Note that there is no difference between this system and traditional systems, where each process knows all other processes.
%     Since solving Byzantine consensus in traditional partially synchronous systems requires at least $2f+1$ correct processes to tolerate $f$ Byzantine faults~\cite{dwork_1988}, the described system also requires at least $2f+1$ correct processes.
%     Therefore, the fact that processes cannot provide false information about the sets received from their PDs has no effect on Property~II.
% \end{proof}

% \subsection{Correctness Proofs for the Discovery Algorithm}\label{appendix:discovery}
% \begin{proof}[Proof of Theorem~\ref{thm:discovery:sink}]
% Consider a system with a knowledge connectivity graph $G_{\mathit{di}} \in \mathcal{G}_\mathit{di}$. 
% Suppose $V_{\mathit{sink}}$ comprises the sink members of $G_{\mathit{di}}$.
% By executing Algorithm~\ref{alg:discovery:known:f}, we need to show that each correct process $i$ eventually
%     \begin{enumerate*}[label=(\alph*)]
%         \item discovers all sink members, i.e., 
%         $V_{\mathit{sink}} \subseteq \mathit{known}$, and
%         % 
%         \item receives the PDs of all correct sink members, i.e.,
%         $V_{\mathit{sink}} \cap C \subseteq \mathit{received}$.
%     \end{enumerate*}
% We divide the proof into the following two cases:
% \begin{itemize}
%     \item Process~$i$ is a correct sink member.
%     Let $d_{\mathit{ss}}$ denote the longest distance between any two correct sink members.
%     After GST, $i$ sends a \textsc{GetPDs} message to its PD members, and each correct process within $\mathit{PD}_i$ responds by sending its PD to $i$.
%     Hence, process $i$ receives the PDs of correct sink processes within a distance of two from itself at most by time $\text{GST} + 2\delta$.
%     It then sends a \textsc{GetPDs} message to the processes within a distance of two from itself, and each correct process that receives such a message responds by sending its PD to $i$.
%     Consequently, it receives the PDs of correct sink processes within a distance of three from itself at most by time $\text{GST} + 4\delta$.
%     Using the same argument, process~$i$ receives the PDs of all correct sink members at most by time $\text{GST} + 2(d_{\mathit{ss}}-1)\delta$, i.e., $V_{\mathit{sink}} \cap C \subseteq \mathit{received}$.
    
%     Note that any Byzantine sink process must be known by at least $f+1$ correct sink members. 
%     This is because there must be at least $f+1$ node-disjoint paths between any two sink members, as stated in Theorem~\ref{thm:sink:alternative:def}.
%     Even if a Byzantine sink member $j$ remains silent, $j \in \mathit{known}$ at most by time $\text{GST} + 2(d_{\mathit{ss}}-1)\delta$, as $i$ receives the PDs of all correct sink members by that time.
%     It follows that $i$ can eventually discover all sink members, i.e., $V_{\mathit{sink}} \subseteq \mathit{known}$.
%     % 
%     \item Process~$i$ is a correct non-sink member.
%     Let $d_{\mathit{ns}}$ denote the longest distance between a correct non-sink member and a correct sink member.
%     After GST, process~$i$ sends a \textsc{GetPDs} message to its PD members, and each correct process within $\mathit{PD}_i$ responds by sending its PD to $i$.
%     Hence, process~$i$ receives the PDs of correct processes within a distance of two from itself at most by time $\text{GST} + 2\delta$.
%     It then sends a \textsc{GetPDs} message to the processes within a distance of two from itself, and each correct process that receives such a message responds by sending its PD to $i$.
%     Consequently, it receives the PDs of correct processes within a distance of three from itself at most by time $\text{GST} + 4\delta$.  
%     Using the same argument, process~$i$ receives the PD of at least one correct sink member~$j$ at most by time $\text{GST} + 2(d_{\mathit{ns}}-1)\delta$, as there are at least $f+1$ node disjoint paths made by correct processes from $i$ to $j$.
%     It follows that $i$ discovers all correct sink members at most by time $\text{GST} + 2(d_{\mathit{ns}} + d_{\mathit{ss}} - 2)\delta$, which means it can eventually discover all sink members, as well receiving the PDs of all correct sink members.
% \end{itemize}
% \end{proof}

% \subsection{Correctness Proofs for the Sink Algorithm}\label{appendix:sink}
% \begin{proof}[Proof of Theorem~\ref{thm:sink:alternative:def}]
%     We divide the proof of this theorem into the following two steps:
%     \begin{itemize}
%         \item If $S$ comprises all sink members, then the three properties identified in Theorem~\ref{thm:sink:alternative:def} must be satisfied.
%         % 
%         \item If the three properties identified in Theorem~\ref{thm:sink:alternative:def} must be satisfied.
%     \end{itemize}
% \end{proof}

% \begin{proof}[Proof of Theorem~\ref{thm:sink:termination}]
%     From Theorem~\ref{thm:discovery:sink} and Theorem~\ref{thm:discovery:non:sink}, any correct process discovers all correct sink members at most by time $t = \mathtt{max}\{\text{GST} + 2(d_{\mathit{ss}} - 1)\delta,\text{GST} + 2(d_{\mathit{ns}} + d_{\mathit{ss}} - 2)\delta\}$.
%     We show that the conditions presented in line~\ref{line:sink:condition} within Algorithm~\ref{alg:sink:known:f} are met at time $t$.
%     As a consequence, any correct process stops to await further, resulting in the termination of the algorithm.
    
%     Since any correct process discovers all correct sink members at time $t$, we have $\forall \ i \in V_{\mathit{sink}} \cap C : V_{\mathit{sink}} \cap C \subseteq \mathit{known}(i)$.
%     Likewise, at time $t$, we have $\forall \ i \in V_{\mathit{sink}} \cap C : V_{\mathit{sink}} \cap C \subseteq \mathit{received}(i)$.
%     Consequently, the two sets $K$ and $S$ specified in the conditions exist such that $\forall \ i \in V_{\mathit{sink}} \cap C : K=\mathit{known}(i)=S=\mathit{received}(i)$.
%     From Definition~\ref{def:osr}, the connectivity of the correct sink members is at least $f+1$.
%     Hence, the connectivity of $K$ and $S$ is at least $f+1$, completing the proof.
% \end{proof}

% \begin{proof}[Proof of Theorem~\ref{thm:sink:sink}]
%     We divide the proof into the following two parts:
%     \begin{itemize}
%         \item Proving the theorem for the sink members.
%         Let $i$ be a correct sink member.
%         Assume process $i$ executes the Sink algorithm and receives $S$.
%         In order to prove this part, we need to show that $S = V_{\mathit{sink}}$.
%         With this aim, we show that $S$ does not contain any non-sink members, and it contains all sink members.
    
%         \vspace{0.5em}
%         \noindent\textbf{\textit{S} does not contain any non-sink members.}
%         For the sake of contradiction, assume $S\setminus V_{\mathit{sink}} \neq \emptyset$.
%         Accordingly, at least one non-sink member $j$ is within $S$.
%         From the definition of the $k$-OSR PD (Definition~\ref{def:osr}), from $i$ to $j$ there cannot be $f+1$ node disjoint paths.
%         However, the Sink algorithm returned $S$ as a set in which there are $f+1$ node disjoint paths between members of $S$, which is a contradiction.
%         Consequently, $S$ does not contain any non-sink members.
    
%         \vspace{0.5em}
%         \noindent\textbf{\textit{S} contains all sink members.}
%         For the sake of contradiction, assume $V_{\mathit{sink}} \setminus S \neq \emptyset$.
%         Assume $V_{\mathit{sink}} \setminus S = R$, where $R$ is a non-empty set with size $r$.
%         From the definition of the $k$-OSR PD (Definition~\ref{def:osr}), there must be at least $f+1$ correct processes that are not members of $R$ and know each process $j \in R$.
%         Since $S$ does not contain $j$, it cannot contain those $f+1$ correct processes, which is a contradiction as the size of $R$ must be at least $r+f+1$.
%         Consequently, $S$ contains all sink members.

%         \item Proving the theorem for the non-sink members.
%         Let $i$ be a correct non-sink member.
%         Assume process $i$ executes the Sink algorithm and receives $S$.
%         In order to prove this part, we need to show that $S = V_{\mathit{sink}}$.
%         With this aim, we show that $S$ cannot be comprised of non-sink members; it does not contain any non-sink members; it contains all sink members.

%         \vspace{0.5em}
%         \noindent\textbf{\textit{S} cannot be comprised of non-sink members.}
%         For the sake of contradiction, assume $S$ is comprised of non-sink members, i.e., $S \subseteq \Pi \setminus V_{\mathit{sink}}$.
%         Since $S$ is returned by the Sink algorithm, it satisfies the conditions presented in line~\ref{line:sink:condition} within Algorithm~\ref{alg:sink:known:f}.
%         We can also assume a set $K$ exists such that $|K\setminus S|\leq f$ and $K \cap V_{\mathit{sink}} = \emptyset$.
%         As there are at least $f+1$ node-disjoint paths made by correct processes from members of $K$ to the sink, $|K\setminus S| \geq f+1$ if $K \cap V_{\mathit{sink}} = \emptyset$, which is a contradiction. 
%     \end{itemize}
% \end{proof}

% \subsection{}

% \begin{proof}[Proof of Theorem~\ref{thm:sink:sink:wf}]
%     Assume the number of disjoint paths between members of $A$ obtained by executing $\mathtt{numPotentialDisjointPaths}(A)$ is $k$.
%     For the sake of contradiction, assume there is another function $\mathtt{F}(A)$ that can estimate the number of disjoint paths between members of $A$ by $k'<k$. 
%     Without loss of generality, assume $k'=k-1$.
%     This means $\mathtt{numPotentialDisjointPaths}(A)$ considers a disjoint path by a silent process $s$ while $\mathtt{F}(A)$ does not consider it.
%     As $s$ is silent, it might be correct and increase the number of disjoint paths between members of $A$. 
% \end{proof}

% \begin{proof}[Proof of Theorem~\ref{thm:sink:non:sink:wf}]
%     We know there are at least $2f+1$ correct processes inside the sink.
%     For the sake of contradiction, assume we can present an estimation $\hat{f}<\floor{(|Q|-1)/3}$.
%     Now consider the following case.
%     The sink is a complete graph with $f$ faulty processes.
%     Hence, $|Q| = |3f+1|$.
%     $\hat{f}<\floor{(|Q|-1)/3} = f$, which contradicts our rule.
% \end{proof}


\end{document}

